In-Medium Similarity Renormalization Group Approach to the Nuclear Many-Body Problem

We present a pedagogical discussion of Similarity Renormalization Group (SRG) methods, in particular the In-Medium SRG (IMSRG) approach for solving the nuclear many-body problem. These methods use continuous unitary transformations to evolve the nuclear Hamiltonian to a desired shape. The IMSRG, in particular, is used to decouple the ground state from all excitations and solve the many-body Schr\"odinger equation. We discuss the IMSRG formalism as well as its numerical implementation, and use the method to study the pairing model and infinite neutron matter. We compare our results with those of Coupled cluster theory, Configuration-Interaction Monte Carlo, and the Self-Consistent Green's Function approach. The chapter concludes with an expanded overview of current research directions, and a look ahead at upcoming developments.

==> fig/srg_toy_flow.tex <==
%!TEX root = ../lnp.tex
\begin{picture}(1.0000,0.8400) 

%%%%% eps file %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\put(0.2000,0.2000){\includegraphics[width=0.8000\unitlength] 
  {fig/srg_toy_flow.pdf}} 

%%%%% x-axis %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\put(0.1200,0.1650){\parbox{0.2000\unitlength}{\centering $0$}} 
\put(0.2150,0.1650){\parbox{0.2000\unitlength}{\centering $\tfrac{\pi}{2}$}} 
\put(0.3100,0.1650){\parbox{0.2000\unitlength}{\centering $\pi$}} 
\put(0.4050,0.1650){\parbox{0.2000\unitlength}{\centering $\tfrac{3\pi}{2}$}} 
\put(0.5000,0.1650){\parbox{0.2000\unitlength}{\centering $2\pi$}} 
\put(0.5950,0.1650){\parbox{0.2000\unitlength}{\centering $\tfrac{5\pi}{2}$}} 
\put(0.6900,0.1650){\parbox{0.2000\unitlength}{\centering $3\pi$}} 
\put(0.7850,0.1650){\parbox{0.2000\unitlength}{\centering $\tfrac{7\pi}{2}$}} 
\put(0.8800,0.1650){\parbox{0.2000\unitlength}{\centering $4\pi$}} 

\put(0.2000,0.1000){\parbox{0.8000\unitlength}
  {\centering $\theta(s)$}} 

%%%%% y-axis %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\put(0.0000,0.2270){\parbox{0.1900\unitlength}{\raggedleft$-1$}} 
\put(0.0000,0.3700){\parbox{0.1900\unitlength}{\raggedleft$-0.5$}} 
\put(0.0000,0.5110){\parbox{0.1900\unitlength}{\raggedleft$0$}} 
\put(0.0000,0.6560){\parbox{0.1900\unitlength}{\raggedleft$0.5$}} 
\put(0.0000,0.7990){\parbox{0.1900\unitlength}{\raggedleft$1$}} 

\put(0.0700,0.2000){{\color{white}.}}
\put(0.0700,0.2000){\begin{sideways}\parbox{0.6400\unitlength}
  {\centering $E_{-}(s),\; V(s)\,[\Omega]$}\end{sideways}} 

%%%%% plot label %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\put(0.2500,0.7400){\parbox{0.7000\unitlength}
  {\raggedleft  }} 

%%%%% user stuff %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{picture} 

